Not All Errors Are Made Equal: A Regret Metric for Detecting System-level Trajectory Prediction Failures

Robot decision-making increasingly relies on data-driven human prediction models when operating around people. While these models are known to mispredict in out-of-distribution interactions, only a subset of prediction errors impact downstream robot performance. We propose characterizing such "system-level" prediction failures via the mathematical notion of regret: high-regret interactions are precisely those in which mispredictions degraded closed-loop robot performance. We further introduce a probabilistic generalization of regret that calibrates failure detection across disparate deployment contexts and renders regret compatible with reward-based and reward-free (e.g., generative) planners. In simulated autonomous driving interactions and social navigation interactions deployed on hardware, we showcase that our system-level failure metric can be used offline to automatically extract closed-loop human-robot interactions that state-of-the-art generative human predictors and robot planners previously struggled with. We further find that the very presence of high-regret data during human predictor fine-tuning is highly predictive of robot re-deployment performance improvements. Fine-tuning with the informative but significantly smaller high-regret data (23% of deployment data) is competitive with fine-tuning on the full deployment dataset, indicating a promising avenue for efficiently mitigating system-level human-robot interaction failures. Project website: https://cmu-intentlab.github.io/not-all-errors/

==> sections/intro_v5.tex <==
\section{Intro}
\label{sec:intro}

Data-driven human models have transformed how robots interact with people in settings ranging from autonomous driving \cite{hagedorn2023rethinking}, to tabletop manipulation \cite{kedia2023interact, kedia2023manicast}, and even game-play \cite{abeyruwan2023sim2real}. 
Despite their widespread adoption, these models are still susceptible to mis-predicting human behavior, potentially causing robots to make unsafe decisions and raising the need for detecting and mitigating such prediction failures.
The predominate approach for quantifying predictor performance is to analyze the model in isolation (i.e., \textit{component-level} analysis). For example, predictor failures can be measured by sufficiently large deviations between the predicted versus real human behavior \cite{sun2021complementing}; in turn, this data   
 %observed during robot deployment is 
% by the robot during deployment is
% the robot using its predictor to interact with humans is 
%mined to find scenarios where the distance between the predicted versus real human behavior was sufficiently large \cite{bla}. \ttnote{This data 
could be used to develop benchmarks, anomaly detectors, or re-train the predictor itself.
While this approach is automatic and easy to implement, it omits the fact that prediction errors at the \textit{component-level} do not always lead to \textit{system-level} robot performance degradation \cite{chen2023treeplanning}, 
For example, in the left image of Figure~\ref{fig:regret}, the parked white vehicle was erroneously predicted to start slowly moving; however, from the blue robot vehicle's perspective, its performance was not impacted by these mis-predictions.
% Scenarios like these are irrelevant: 
Consequently, a predictor does not need to waste its limited capacity being re-trained on such mis-predictions, and anomaly detectors should not unnecessarily activate. 
% \ttnote{especially when the capacity of the prediction model is limited for real-time feasibility}. 
However, automatically detecting such system-level prediction failures from human--robot interaction data requires a system-level metric that rigorously quantifies the impact of prediction failures on robot decisions.

% \new{We generalize the canonical notions of regret to introduce a system-level metric for automatically identifying system-level prediction failures. This metric is a first step toward scalable analysis and auditing of human prediction models, and we demonstrate the use of the data identified by our metric with prediction fine-tuning a conditional behavior prediction model in the autonomous driving setting.}

\new{In this work, our key insight is that system-level human prediction failures are} precisely characterized by the mathematical notion of \textit{regret}. Canonically, regret measures the difference between
% \todo{Consequently, treating every prediction failure equally during predictor improvement will not only increase the training costs but also potentially degrade the model's performance in critical scenarios due to its limited capacity.}
\new{the maximum reward decision in hindsight}
% between the maximum reward that the robot could have achieved 
given complete information and the realized reward from its actual decision made under uncertainty \cite{zinkevich2003online}.
\new{In theory, identifying all deployment interactions with sufficiently high regret would automatically extract all system-level prediction failures.}
% \new{Unfortunately, in practice} the standard regret definition is poorly calibrated for consistently identifying such failures across diverse deployment contexts where 
% \new{the achievable reward distribution} varies significantly 
% (e.g., stuck in gridlock versus open-road driving). 
% While regret is a principled measure, 
Unfortunately, the standard regret definition can be poorly calibrated across disparate deployment contexts. This is because the reward gap between the hindsight-optimal decision and executed decision varies widely between different deployment contexts (e.g., sparse versus crowded highway driving).
Thus, we propose that
\begin{quote}
    % \textit{high regret interactions are those in which human mis-predictions significantly impacted robot decision-making, and yeild the most training signal for improving the robot's overall performance.}
    % \textit{high regret scenes characterize interaction-relevant prediction failures, and yield the most training signal for improving the robot's overall performance.}
    \centering
    % \textit{%mapping regret to probability space %
    % mapping regret to \textbf{probability space} calibrates anomaly detection between disparate contexts.}
    %\textit{\new{evaluating the quality of a robot decision by its likelihood rather than its absolute reward calibrates regret across disparate contexts.}}
    \textit{\new{regret is a rigorous measure for automatically identifying \\ system-level human prediction failures.}}
    %mapping regret to probability space  enables \\calibrated detection of interaction failures\\ between disparate contexts.}
\end{quote}
\new{This idea is inspired by mathematical psychology and econometrics, wherein an agent's decisions are interpreted as noisily-optimal under some reward, normalized by the reward of alternative decisions in that context \cite{luce2005individual, baker2009action}.
It is precisely this normalization that calibrates the perceived quality of a decision relative to the context-dependent reward scale. 
Thus, even if two contexts have wildly different reward scales (e.g., sparse versus crowded highway), a likelihood model is a principled way to place all decision comparisons on the \textit{same} scale: a value between zero and one.}
% (e.g., the scale of the reward in sparse highway is smaller than the crowded one because less reward features are active).}}
% When comparing the quality of an agent's decisions in two \textit{different} contexts , 
% places all in context-reward scale.}}
% changes as a function of the context (e.g., sparse versus crowded highway),
%To this end, 
\new{With this probabilistic model}, we derive a calibrated regret metric 
that enables meaningful comparisons of how prediction failures degrade closed-loop human-robot interaction performance across diverse deployment contexts. 
\new{Moreover, since our regret metric only requires evaluating decision quality via likelihoods instead of direct rewards, we} generalize the use of regret for \new{reward-free robot interaction planners, such as generative neural planners \cite{seff2023motionlm}}. 
% (e.g., with generative planners that do not use explicit reward functions).  
%is immediately compatible with neural generative planners that do not model explicit rewards (as required in traditional definitions of regret). 

% We argue that regret is a good metric for evaluating prediction failures because it calibrates the severity of anomalous interactions to the robot's planning ability: 
% via regret, we can calibrate the severity of anomalous interactions to the robot's planning ability, focusing on the ``best the robot could have done'' in hindsight, now that the true human behavior was revealed. If mis-predictions were truly irrelevant to the robot's task at hand, then even after observing the true human behavior, the robot would have made the same decision. Conversely, interaction-relevant prediction failures induce high robot regret, as the robot realized it could have made a safer or more performant decision now that it knows how the human truly behaved. 

% this metric isolates the data that improves closed-loop interaction the most even with 77\% less total data 

\new{In a series of} closed-loop simulation experiments in the autonomous driving domain, we \new{automatically extract high-regret human-robot interaction data, revealing flawed aspects of the human prediction model that lead to system-level robot failures (e.g., a false sense of influence and a misunderstanding stranded agents, shown on the right of  Figure~\ref{fig:regret})}.
% Finally, we \new{leverage our 
%To study this, we fine-tune the robot's predictive model only on these high-regret scenarios, comparing against other subsets of the deployment dataset (such as random selection, or only low-regret interactions). 
% We study this by conducting closed-loop simulation experiments in the autonomous driving domain, 
\new{We further investigate} the value of this high-regret data for improving a robot's downstream decision-making. We find that fine-tuning the robot's \new{human behavior} predictor on a small subset ($23\%$) of the total deployment data yields consistent improvements during robot re-deployment when the subset contains only high-regret data, unlike other possible subsets such as a random selection or only low-regret interactions.
%so long as the dataset is comprised entirely of high-regret interactions. 
Furthermore, fine-tuning on high-regret data is competitive with the performance improvements achieved by fine-tuning on the full dataset and does not exhibit any degradation artifacts in nominal interaction settings.
%that fine-tuning with only the top $p=20$-quantile of high-regret interactions---which constitutes $23\%$ of our deployment data---can yield the best closed-loop robot performance improvements in all validation simulations, while all other dataset splits cause inconsistent performance changes.  
% so long as the data captures the interaction-relevant failures
\new{Ultimately, our analysis reveals that} the very presence of \new{high-regret} data during \new{human behavior} predictor fine-tuning is one of the most important indicators of downstream robot \new{decision-making} improvement. 
% In fact, fine-tuning on datasets that have little or no interaction-relevant failure data cannot .....

\new{While we take a first step towards continually improving robot interactions with people, our \textbf{core contribution} is a general} regret-based data selection approach \new{for automatically identifying system-level prediction failures \cite{sinha2022system}. Beyond our demonstration of behavior predictor fine-tuning, our approach suggests several interesting directions for future work, including using historical data of system-level prediction failures to construct runtime monitors and automatically explaining the semantics of the failures themselves.} %he use of this metric is not limited to only improving specific modules of the autonomy stack, but can also add explainability for how and when complex autonomous systems fail.} 


%In addition to this being a new insight into \new{how to detect and learn from 
% what kind of prediction training data can give value to 
%system-level failures induced by mis-predictions \cite{sinha2022system}}, 
%our regret-based data selection approach \new{shows a promising first step towards} mitigating human-robot interaction failures at-scale. 






==> sections/method_old.tex <==
\section{A Calibrated \new{Regret Metric} for \new{Detecting} 
% Interaction-Relevant 
\new{System-Level} Prediction Failures}
\label{sec:method-failure-detection}

Our core idea to detect 
% interaction-relevant prediction failures (IPF) 
\new{system-level} prediction failures 
is grounded in the notion of \textit{regret}: high-regret interactions are those in which incorrect human predictions negatively impacted robot decision-making. 
Intuitively, by ranking all the human-robot trajectory data from $\data$ by the robot's deployment regret, we can quantify the most anomalous interactions from the perspective of the robot.
% \todo{HEY WE DO THIS FOR COST AND GENERATIONS!}
% relies on formalizing a notion of regret. 
% \todo{[example?]}


% \para{Deriving Calibrated Regret from Reward-based Planning} 
\para{Regret Calibration Challenges in Reward-based Planning}
The canonical measure of regret is defined in reward space and considers the difference between the maximum possible reward that the robot could incur \textit{in hindsight} and the realized reward from its actual decision \cite{zinkevich2003online}.
However, even with a reward-based planner in which the rewards are readily queryable, directly using the canonical measure of regret may not \new{always} rank interactions in a desired way. 
This is because an underlying assumption in this definition is that the reward is perfectly calibrated between deployment scenarios or contexts, making two high-regret interactions from different deployment contexts directly comparable. 
% these traditional applications of regret typically assume static settings where the reward distribution remains the same between scenarios. 
Unfortunately, in practice, when robots are deployed in a wide variety of scenarios and contexts $\context$, it is extremely hard to have such a perfectly calibrated reward, complicating the straightforward application of absolute reward-based regret for failure detection. We illustrate this technical point with a \new{representative} example \new{drawn from our simulation experiments (details in Section \ref{sec:experimental-setup})}. 
% reward distribution over robot actions can vary dramatically, which complicates this traditional notion of regret. 


\para{\textit{Illustrative Example}} \textit{Consider the first column of Figure \ref{fig:regretExample}, where the same robot is deployed in two different contexts: one where the robot drives \new{behind a stopped truck} (\new{$C_1$}) and the other where the robot \new{approaches an intersection} (\new{$C_2$}). 
The robot's reward function is a linear combination of control effort, collision penalty, \new{road progress, and lane-keeping.} 
%In both scenarios, the robot has the same two decisions to choose from: quickly change to the left lane (\new{curved} trajectory), which always incurs a small control effort cost $-\delta, ~|\delta| \ll 1$,  or proceed forward (\new{straight} trajectory), which always incurs no control cost. 
%Assume in scenario A the robot chooses to change lanes, and in scenario B it chooses to proceed forward. 
\new{In scenario $C_1$, the robot mispredicts the stopped truck begins moving and initiates a lane change, and in scenario $C_2$, it takes an aggressive maneuver to avoid nearby traffic.}
\new{The reward distribution of the executed and hindsight-optimal action in each scenario is shown on the right of Figure \ref{fig:regretExample}.} A traditional regret metric assigns scenario \new{$C_1$ a regret of $11.4$ and $C_2$ a regret of $11.7$.}
%A traditional regret metric assigns scenario A a regret of $\delta$ (induced by the inefficient lane change) and assigns scenario B a $100 - \delta$ regret due to the collision proximity cost that was never active in the other scenario. 
\new{However, it is only in scenario $C_1$ where the suboptimal behavior led to the robot taking an extremely poor action. In reality, despite $C_2$ taking an unnecessarily aggressive action, the robot was able to safely proceed through the intersection. While the robot could have taken a more optimal action in both scenarios, canonical measures of regret are unable to identify scenario $C_1$ as being a worse decision in that context.} 
% We desire a properly calibrated regret metric that would incur a high regret for the suboptimal action in both scenarios. However, without designing a complex, context-dependent reward function for the robot, it is impossible to calibrate traditional notions of regret to fairly compare 'poor actions' across different scenarios.
}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/Illustrativev3.png}
    \caption{\textbf{Illustrative Example.} \new{Left column shows the robot's predictions and deployment-time decision. Right column shows the counterfactual analysis given observed human behavior. Top Row ($C_1$): The robot mispredicts a stopped vehicle to begin moving and chooses to change lanes. In reality, the truck remained stopped. Bottom Row ($C_2$): The robot mispredicts a stopped car to stay stopped and swerves offroad to avoid a collision. The human's executed actions instead drove forward.} Canonical measures of regret rate scenario \new{$C_1$ as equivalent to $C_2$, even though the robot's behavior $C_1$ led to qualitatively worse behavior. Each hindsight-optimal action and executed action's reward is shown on the right scale.}}
    \label{fig:regretExample}
\end{figure}

%\begin{figure}[t!]
%    \centering
%    \vspace{-0.5em}
%    \includegraphics[width=\linewidth]{figures/illustrative_alt.png}
%    \caption{\textbf{Illustrative Example.} \new{The} robot can go straight or change lanes. An unnecessary lane change incurs a control effort penalty $-\delta$ (left).  Driving too close to the deer activates a collision penalty of $-100$ not present in scenario A (right). Canonical measures of regret rate scenario B much worse than scenario A, even though they were both poor decisions in their respective contexts.}
%    \vspace{-1em}
%    \label{fig:regretExample}
%\end{figure}

\para{A General Calibrated Regret Metric}
To appropriately account for the context-dependent reward distributions, \new{we propose that during regret computation, decision quality should be evaluated in probability-space.}
That is, instead of looking at the \textit{absolute} robot reward, we consider the reward of a candidate decision \textit{normalized} by the reward of all other possible decisions in that scenario. 
Specifically, we utilize a likelihood model that can compute the counterfactual probability of any candidate robot action sequence, $\aRtraj$, given the \textit{observed} actions of the other human agents, $\aHtrajObs$, and the observed joint state trajectory $\strajobs$ in that context $\context$: 
\begin{equation}
\label{eq:cfprob}
    P_\phi(\aRtraj \mid \aHtrajObs, \strajobs, \context).
\end{equation}
% When the robot originally executed $\aRtrajObs$ it did not have knowledge of the future behavior of the non-ego agents $\aHtrajObs$. It could only use its prediction resulting from $\pred$. In contrast, $P_{\phi}$ serves as an indicator of the quality of the ego's true action relative to any other action it could have taken \textit{in hindsight}, with knowledge of how the other agents actually behaved. 
By normalizing over alternative options in the scene, 
% this conditional likelihood model places all scene evaluations between $[0,1]$, and 
this likelihood model enables fairer comparison of executed robot behaviors, $\aRtrajObs$, across different scenarios irrespective of the absolute reward the robot incurred. 
Note that here the likelihood model shares the same parameters as the robot's planner ($\phi$). For example, if the robot is using a reward-based planner, then this probability distribution is shaped according to the same reward weights and features that the robot uses for decision-making. 
%One exciting consequence of our probability-based approach is that is generalizes a notion of calibrated regret to be readily compatible with generative neural planners. 
%Here, the conditional probability $P_\phi$ can be naturally approximated via querying the generative planner \cite{seff2023motionlm}. With the rise of these types of models in robotics domains, we see this as an important step towards uniting core decision-theoretic concepts with increasingly powerful planning paradigms. 
% In the context of the generative model-based neural planner, 
% \footnote{}.

%\todo{weave this in....Although not the focus of this work, an added benefit of computing regret in probability space is its compatibility with generative robot planners which simultaneously do prediction and planning without an explicit cost function. In the generative model setting, parameters $\phi$ and $\theta$ are equivalent. In this setting, our metric simply requires an approximation of the probability density function that the robot actions are being sampled from.}




%\ttnote{I am not sure if we should use GT actions or predicted actions of the surrounding non-ego agents, like in the context of generative model, you train the model with GT actions, but when you do the generation to get the joint prob, the get the conditional prob, the actions are predicted. In the context of cost based planner, we always use predicted actions?}This is not a strong assumption since any cost-based planner can automatically approximate this using, say, the Luce-shepard model (example in Results). This also applies to any generative planner that can approximate this conditional probability.

%It may be tempting to characterize the interaction-relevant failures by actions that have low conditional probability. However, this neglects that in the presence of multiple, equally good actions, the probability mass would be split between these actions making comparisons difficult to make. \knnote{need to explain this distinction more carefully, or delete.} Instead, we define regret as: \todo{this is treating actions as trajectories rather than per-timestep regret and averaging. double-check this}

% Armed with this conditional likelihood model, 
For any deployment scenario $d \in \data$,  we quantify the deployment regret at timestep $t$ as: 
\begin{equation}
\begin{aligned}
        \regret_t(d) := \max_{\aRtraj_t} &\big[P_\phi(\aRtraj_t \mid \aHtrajObs_{t}, \strajobs_{t}, \context)\big] - P_\phi(\aRtrajObs_{t} \mid \aHtrajObs_{t}, \strajobs_t, \context).
        \label{eq:regret}
\end{aligned}
\end{equation}       
Intuitively, if the other agents behaved exactly as the robot's model $\pred$ expected, then the robot would have executed a trajectory deemed high-performance that incurs low regret. 
More subtly, if the predictions failed to capture human behavior in a way that was 
% if the behavior of other agents deviated in ways that are 
\textit{irrelevant} to the robot's performance, 
% (e.g., unexpectedly turning away from the robot's planned trajectory), 
then the robot's executed trajectory will \textit{still} have low regret. 
% since the unexpected behaviors of the other non-ego agents did not prevent the ego agent from successfully performing its task. 
Ultimately, the robot will only have a high regret if its planner was blindsided by a mis-prediction that impacted its ability to execute a high-performance trajectory. 

\para{\textit{Illustrative Example}} \textit{Going back to the reward-based planning setting in Figure~\ref{fig:regretExample}, let us define the probability of each robot decision using the Luce-Shepard choice rule \cite{luce2005individual}, \new{which places exponentially more probability on robot decisions that are high-reward under its  reward function.} \new{Recall that the canonical regret metric evaluated the unnecessarily aggressive (but safe) maneuver in $C_2$ as approximately the same regret as the  unsafe lane change into a stopped truck in $C_1$. 
% Although the canonical regret metric for the 
% unnecessarily aggressive maneuver is slightly higher in $C_2$ than the regret of the unsafe lane change in $C_1$, 
In contrast, our calibrated regret metric, which evaluates the decision likelihood of each action, results in an intuitive separation: $C_1$ has a higher regret of $0.56$ compared to $0.34$ in $C_2$.}%It is a simple exercise to show that our regret metric assigns scenario A's suboptimal actions a regret of $\frac{\exp(0)-\exp(-\delta)}{\exp(0)+\exp(-\delta)} \approx 1-\delta$ and scenario B's suboptimal actions a regret %$\frac{\exp(-\delta)+\exp(-100+\delta)}{\exp(-\delta)+\exp(-100+\delta)} \approx 1-\delta$
%$\frac{\exp(-\delta)-\exp(-100)}{\exp(-\delta)+\exp(-100)} \approx 1-\delta$, capturing comparable levels of anomalous decisions.
}

\para{\new{Extracting High-Regret Interactions} ($\data_\mathcal{I}$)} Finally, leveraging our general calibrated regret metric from Equation~\ref{eq:regret}, we score each scene $d \in \data$ by taking the average of the per-timestep regrets\footnote{Additional variants for computing the total regret of a scene are explored in the supplementary material.}. 
Akin to Farid et al. \cite{farid2023task}, we utilize these rankings to form an empirical regret distribution and pick the top $p$-quantile of scenarios with highest regret to constitute our \new{system-level failure} dataset, $\data_\mathcal{I}$, where $p$ is a design choice.
In Figure~\ref{fig:regret}, we visualize a histogram of the deployment regret distribution extracted from our closed-loop autonomous-driving simulation experiments, demonstrating the infrequent but high-regret nature of system-level prediction failures (more details in Section~\ref{sec:results}). Interesting scenarios emerge as high-regret, such as the robot believing it can influence stopped traffic to start moving if it starts driving \new{(Figure \ref{fig:regret}, middle)}, or being unable to understand how a stranded truck will not move out of the way \new{(Figure \ref{fig:regret}, right)}. 
\new{For further comparisons on the differences between the scenarios extracted by our metric and prior approaches such as L2 prediction error, canonical regret, and the approach from Farid et al. \cite{farid2023task}, please refer to the supplementary Section~\ref{app:metric-comparisons}. }

%%%%%%%%%%%

% \section{Learning to Predict Interaction Failures \\ for Deployment Improvement}

\section{Learning to Predict High-Regret Interactions for Deployment Improvement}
% attending to interaction failures for robot improvement 
% \section{Continually Improving \\ Robot Interaction with People}
\label{sec:method-finetuning}


% * we have a metric, but we also want the robot to get better
% * since the core reason the robot failed was because it didn't understand influence, lets focus on improving its predictive model
% * we could just finetune with everything, but our regret metric just revealed that only a subset of mis-predicted human behaviors / interactions mattered for the "closed-loop" robot performance
% * this may indicate that we shouldnt waste the prediction model's capacity by treating every datapoint as equal when we retrain, which would only increase training cost and may lead to unexpected model changes in critical scenarios  
% * in fact, we hypothesize that the scenes we identified with our regret metric are precisely the interactions that our model was \textit{missing}. 
% * In other words, \textit{if the predictor is unable to understand what action may lead to poor interaction outcomes, the planner will incorrectly evaluate which actions it should avoid.}
% * we investigate fine-tuning the prediction model just on the IPF data, 

Thus far we have proposed a calibrated detection method for identifying \new{system-level prediction} failures, but we are also interested in the potential for robot performance improvement.
Here, the fundamental challenge is that the robot has an incomplete understanding of how its behavior may influence other agents. 
One approach could be to retrain (or fine-tune) the prediction model $\pred$ on all the recorded deployment data, $\data$. However, our regret metric just revealed that only a subset of mis-predicted human behaviors and robot interactions really mattered for closed-loop robot performance. As a result, this may indicate that the prediction model's limited capacity should not be wasted by treating every data point as equal. Treating all data as equally valuable would only increase training costs as the size of $\data$ grows and could lead to unexpected model changes in critical scenarios. 
In fact, we hypothesize that the scenarios we identified with our regret metric, $\data_\mathcal{I} \subset \data$, are precisely the interactions that the robot's predictive model was missing.  
In other words, \textit{if the robot's predictor cannot understand what robot actions can lead to poor interaction outcomes, the planner will be unable to evaluate which actions to avoid.}
\new{By focusing the model on learning to predict high-regret interactions, we hypothesize this will enable} the model to expand its understanding of how the interaction could evolve (even if it leads to undesirable outcomes) and at re-deployment time, the robot can actively steer away from these possibilities.
% incorrectly evaluate which actions it should avoid.
In Section~\ref{sec:experimental-setup}, we detail a straightforward approach for incrementally improving robot performance by fine-tuning its prediction model $\pred$ on only the system-level failure dataset $\data_\mathcal{I}$. 


%This regret characterizes the difference between the conditional probability of the best action the robot could have taken given the ground-truth behavior of the other vehicles and its ground-truth action. This is computed per timestep and averaged over the time horizon. Alternative flavors of this regret metric are explored in the supplementary materials. 
% In order for a robot to effectively interact with people,
% after observing the true as a result of deployment around true agent behavior. 
% Since the robot's deployment degradation is so heavily impacted by mis-predictions of human behavior, 
% In order for the robot to improve its real-world interaction performance, 
% in order to improve its long-term deployment performance, it must complete its understanding of the coupling between its behavior and other agents'. 
% how its behavior may influence others. 
% Unfortunately, since the large datasets a robot's predictor is typically trained and evaluated on only contain examples of `good' interaction, the predictor often learns to only predict 'good' effects that lead to good interactions.
% Our regret metric revealed that only a \textit{subset} of the interaction data and mis-predicted human behaviors 

% For example, in driving training and validation datasets, collisions are almost never observed. 
% As a consequence, conditional prediction models often include a loss function that penalizes predicting collisions during training  \cite{chen2023treeplanning, tolstaya2021identifying}. But this means that the robot will have a poor understanding of what behavior leads to undesirable outcomes. However, during deployment, the ability to accurately predict poor interaction outcomes is critical for downstream planning. 
% \textit{If the predictor is unable to understand what action may lead to poor interaction outcomes, the planner will incorrectly evaluate which actions it should avoid. }
% Then, one key aspect to improving robot performance over time is to improve the predictor's performance on scenarios whenever a bad prediction leads to poor interaction performance. We propose doing this by finetuning the prediction model using the interaction-relevant failure data: this lets the model expand its understanding of how the interaction could evolve---even if it leads to undesirable outcomes---and at deployment time, the robot can steer away from these possibilities.
% The implementation details of the finetuning depend on both the architecture of the predictor and the amount of available data for finetuning. Previous works have finetuned the entire predictor \cite{bla}, the last layers of the predictor \cite{bla}, or specific submodules of the predictor \cite{bla}. The critical aspect of our approach is that this finetuning is done on $\datai$, the interaction-relevant subset of the deployment data.



==> sections/results_old.tex <==
\section{Experimental Setup}
\label{sec:experimental-setup}

To evaluate the potential of our approach in data-rich human-robot interaction deployment contexts, we ground our experiments in driving interactions between an autonomous vehicle and human-driven vehicles. Here we detail the specifics of our robot planner, human predictor and associated fine-tuning methodology, and state-of-the-art simulator which enables us to test closed-loop ``deployment'' of the robot under different controlled conditions. 

% \abnote{Instead of just diving into the results, we could also pose certain hypotheses here, similar to what we did in Thomas's recent ICLR paper. (e.g., some ideas: \textbf{H1.} \textit{Re-training the behavior predictor on task-relevant failures improves downstream robot safety and performance.}, \textbf{H2.} \textit{Improvments in average ``population-level'' prediction accuracy does not imply improvements in planning performance.}. For each hypothesis, we write down what the experimental setup was, what we measured, and the results. ) An alternative framing instead of hypotheses is ``findings''. }

% \subsection{Setup}
\para{\new{Robot Policy:} Tree Policy Planning (TPP)} Our planner $\pi_\phi$ is a tree-structured contingency planner developed by Chen et al. \cite{chen2023treeplanning}. This reward-based planner is compatible with state-of-the-art conditional behavior prediction models to account for the influence of the robot's actions when planning. 
The planner first generates a tree of randomly sampled multi-stage dynamically feasible trajectories, after which each branch is fed into an ego-conditioned predictor $\pred$ to generate a scenario tree comprised of multimodal predictions. 
The optimal robot trajectory is obtained by maximizing a hand-designed reward function \new{which is a linear combination of collision costs, lanekeeping costs, control costs, and distance-traveled reward} (full details can be found in the original paper \cite{chen2023treeplanning}). \new{This reward function is fixed throughout the entire robot deployment and human predictor fine-tuning process.}

\para{Base \new{Human} Predictor} 
For our prediction model $\pred$, we train an ego-conditioned variant of the state-of-the-art Agentformer model \cite{yuan2021agent} where the context $\context$ is the semantic map. 
The training loss is a weighted sum of three terms: $1)$ prediction loss that penalizes incorrect predictions from the ground truth, $2)$ ego-conditioned collision (EC) loss that penalizes collisions between the predictions and conditioned ego-action. $3)$ other regularization losses such as diversity and KL divergence loss. 
Our base prediction model is trained on the Nuscenes dataset \cite{caesar2020nuscenes}, consisting of 1,000 20-second driving logs collected in Boston and Singapore. During this phase of training, we use a learning rate of 1e-4. 
% learning rate of $1e-4$ on , a dataset of 1000 20-second driving logs collected in Boston and Singapore. 

\para{Fine-tuning the Predictor}
For fine-tuning, we unfreeze only the last 1.5M parameters of the 17.7M parameter Agentformer model. 
This corresponds to the last half of the future decoder module \cite{yuan2021agent}. 
Across all our baselines, we fine-tune the predictor to see the data for 25 epochs at a reduced learning rate of 5e-5 held constant throughout the 25 epochs. Furthermore, when fine-tuning we eliminate the diversity loss and EC collision loss, focusing the model's efforts to only accurately predict the ground-truth deployment data. \new{Due to the large size of the Nuscenes data, we trained on two Nvidia A6000 GPUS with a batchsize of 14 (effective batch size 28) and gradient accumulation of 5 steps.}

\begin{table}[t]
\centering
% \caption{Post Fine-tuning Open-loop Prediction Performance}
  \begin{tabular}{l|llllllll}
\toprule
\cellcolor[HTML]{D7D7D7} &\multicolumn{3}{c}{\new{ADE / FDE ($\downarrow$)}} \\
 \cellcolor[HTML]{D7D7D7} Fine-tuning Data & Nuscenes & High-Regret & Low-Regret&  \\ \midrule
\multicolumn{1}{l|}{None (Base model)}     & 0.371 / \textbf{1.919}  & 0.639 / 2.999  & 0.610 / 2.375 \\ \midrule 
\multicolumn{1}{l|}{Low-regret-FT} & \new{0.353 / 1.554} & \new{0.386 / 2.333} & \new{0.386 / 1.783} \\ %& 0.367 / 1.578  & 0.395 / 2.359 & 0.391 / 1.755    \\
\multicolumn{1}{l|}{Random-FT}& \new{\textbf{0.315 / 1.435}} & \new{0.366 / 2.100} & \new{0.382 / 1.738} \\   %& \textbf{0.308} / 2.864  & 0.361 / 2.095          &  \textbf{0.370} / \textbf{1.737}             \\
\multicolumn{1}{l|}{High-regret-FT} & %0.332 / 1.928  & \textbf{0.353} / \textbf{2.048} & 0.379 / 1.749      \\ 
\new{0.327 / 1.520} & \new{\textbf{0.333  / 2.014}} & \new{\textbf{0.366/1.713}} \\
\multicolumn{1}{l|}{All-FT} & \new{\textit{\textbf{0.297 / 1.381}}} & \new{\textit{\textbf{0.326 / 1.973}}} & \new{\textit{\textbf{0.340 / 1.665}}}%\textit{\textbf{0.286}} / \textit{\textbf{1.342}}  & \textit{\textbf{0.329}} / \textit{\textbf{1.990}} &\textit{\textbf{0.336}} / \textit{\textbf{1.612}} 
\\ \midrule
\end{tabular}
\caption{\textbf{Fine-tuned Open-loop Prediction Performance.} Average ADE / FDE of the base prediction model and the fine-tuned models on log-replay data. Columns of table indicate different log-replay validation data splits: original Nuscenes data, closed-loop simulation data that exhibited system-level failures (i.e. high-regret), and closed-loop simulation data identified as low-regret. Lowest error is denoted in italics-bold, and second lowest in bold. \new{Each baseline was trained with three random seeds. The reported numbers come from the model with the lowest High-regret ADE/FDE.}}%\abnote{put a little "ADE / FDE ($\downarrow$)" notation underneath Nuscenes + High-Regret + Low-Regret}}
\vspace{-1em}
\label{tab:OL-ade-fde}
\end{table}




\para{Closed-loop Simulation}
In our setting, it is insufficient to simulate human agents using log replay from the original Nuscenes data, since we are specifically looking to identify prediction failures that are coupled with the robot's decision-making.  
% To properly evaluate the impact of the robot's ego-conditioned predictor on downstream decision performance, 
As such, human agents must be allowed to react to the robot's actions, which will inevitably differ from the original driving logs. 
To capture this, we use the state-of-the-art BITS simulation environment \cite{xu2023bits} and use 100 held-out scenes from the original Nuscenes dataset (not used during training) to initialize each simulation.
All non-ego agents are simulated with the off-the-shelf BITS policy, which generates short-horizon goal locations for the agent and corresponding trajectories via reward-based action selection. 
% This simulator was chosen due to the diverse behavior exhibited compared to standard IDM models of simulating traffic \todo{find IDM citation}. 
We constructed the closed-loop deployment dataset $\data$ by running simulations for an interaction horizon of 20 seconds in each of the 100 held-out Nuscenes initializations, matching the length of each scene in the Nuscenes dataset.

\para{\new{Calibrated} Regret Computation} Our regret metric requires access to a conditional probability distribution over robot trajectories \new{given observed human behavior.} \new{Since this case study considers a reward-driven planner, our likelihood model follows from} the Luce-Shepard choice rule \cite{luce2005individual} where the parameters $\phi$ denote the weights of the reward function: 
\begin{equation}\begin{aligned}
P_\phi(\aRtraj_t \mid \aHtrajObs_{t}, \strajobs_{t}, \context) = \frac{1}{Z}e^{R_\phi(\aRtraj_t, \aHtrajObs_{t}, \strajobs_{t}, \context)}, 
\end{aligned}\end{equation}
where $Z := \sum_{\aRtrajAlt_t} e^{R_\phi(\aRtrajAlt_t, \aHtrajObs_{t}, \strajobs_{t}, \context)}$. 
At each timestep in scene $d \in \data$ where the robot originally replanned, %\knnote{should we formally define when replanning occurs in the problem formulation?}
we re-compute the reward of each candidate ego action with respect to the \textit{ground truth} behavior of the other agents, instead of predictions. This allows us to compute the conditional probability of each candidate ego action and obtain the scene's regret $\regret_t(d)$. 



\para{Dat\new{a}set Construction}
Using the deployment dataset $\data$, 
% collecting a deployment dataset of 100 closed-loop simulations in the BITS environment, 
we discarded four due to the absence of non-ego agents, resulting $N=96$ total closed-loop deployment scenarios each of length $20$ seconds. 
We ranked the ego agent's average regret and chose the top $p=20$-quantile\footnote{The percentage of the deployment data to be deemed as \new{system-level} failures is a design decision. 
We chose $p=20$ in part due to the small size of the closed-loop deployment dataset.} of scenarios to be our set of scenes that suffered from interaction-relevant prediction failures, yielding a total of 20 high-regret scenarios in $\datai$. The rest of the 76 scenarios were deemed sufficiently low-regret. 
We hold out 20\% of both high-regret $\datai$ and low-regret $\data \setminus \datai$ scenes (3 and 17 respectively). 
% Of these scenes, we set aside a simulation-validation set comprised of 3 interaction-relevant scenes and 17 interaction-irrelevant scenes. 
The remainder of the deployment data is used for fine-tuning the model. 



\section{Experimental Results}
\label{sec:results}
To investigate how learning to predict high-regret interactions can improve the robot's behavior, we perform a series of experiments wherein we fine-tune the predictive model $\pred$ with different subsets of the deployment dataset, $\data$, and then \textit{re}-deploy the robot in our simulation environment to measure its changes in closed-loop performance. 
Specifically, we hold the robot's planner constant and we redeploy the robot in the simulator on initializations of the held-out 20 validation scenarios (consisting of 3 high-regret scenes and the rest of the 17 as low-regret scenes). 
Importantly, since the behavior of the robot changes as a function of its predictive model in the closed-loop simulation, we once again allow the non-ego agents to respond to the robot via the BITS simulation model.  
% To do this, we simply redeploy the planner and predictor in closed loop simulation initialized using the same 20 Nuscenes data corresponding to the 20 scenes in the simulation validation dataset. \knnote{idt this makes any sense. revise}

\begin{table*}[t!]
\centering
\resizebox{\columnwidth}{!}{
  \begin{tabular}{l|lll|lllll}
\toprule
&\multicolumn{3}{c|}{High-Regret Scenarios} & \multicolumn{3}{c}{ Low-Regret Scenarios}\\ 
  Fine-tuning Data &  Col Cost ($\downarrow$) & Col Severity ($\downarrow$) & Regret ($\downarrow$) & Col Cost ($\downarrow$) & Col Severity ($\downarrow$) & Regret ($\downarrow$)  \\ \midrule
\multicolumn{1}{l|}{\new{Base Model}} &  \cellcolor[HTML]{D7D7D7} \new{10.829} &  \cellcolor[HTML]{D7D7D7} \new{0.848}   & \cellcolor[HTML]{D7D7D7} \new{0.034} &  \cellcolor[HTML]{D7D7D7} \new{\textbf{0.411}} &  \cellcolor[HTML]{D7D7D7} \new{\textit{\textbf{0.051}}}  & \cellcolor[HTML]{D7D7D7}  \new{\textbf{0.006}}    \\ 
\multicolumn{1}{l|}{Low-regret-FT} &\cellcolor[HTML]{c4f2cb} \new{7.489 ($\pm$ 0.408)} & \cellcolor[HTML]{c4f2cb} \new{0.794 ($\pm$ 0.059)} & \cellcolor[HTML]{c4f2cb} \new{0.019 ($\pm$ 0.002)} & \cellcolor[HTML]{fccaca} \new{0.670 ($\pm$ 0.206)}  & \cellcolor[HTML]{fccaca} \new{0.354 ($\pm$ 0.493)}   & \cellcolor[HTML]{fccaca} \new{0.009 ($\pm$ 0.000)}     \\ 
\multicolumn{1}{l|}{Random-FT}            & \cellcolor[HTML]{c4f2cb}{ \new{7.209 ($\pm$ 0.883)} }& \cellcolor[HTML]{c4f2cb}{ \new{0.743 ($\pm$ 0.064)} } &  \cellcolor[HTML]{c4f2cb}{ \new{\textbf{0.016 ($\pm$ 0.003)}} }  & \cellcolor[HTML]{fccaca}{ \new{0.495 ($\pm$ 0.213)} } & \cellcolor[HTML]{fccaca}{ \new{0.076 ($\pm$ 0.054)} } &  \cellcolor[HTML]{c4f2cb}{ \new{\textbf{0.006 ($\pm$ 0.000)}} }             \\
\multicolumn{1}{l|}{High-regret-FT} & \cellcolor[HTML]{c4f2cb} \new{\textbf{3.763 ($\pm$ 0.965)}}  & \cellcolor[HTML]{c4f2cb} \new{\textbf{0.588 ($\pm$ 0.101)}}  & \cellcolor[HTML]{c4f2cb} \new{\textbf{0.016 ($\pm$ 0.003)}}  & \cellcolor[HTML]{c4f2cb} \new{\textit{\textbf{0.397 ($\pm$ 0.814)}}}  & \cellcolor[HTML]{fccaca} \new{0.062 ($\pm$ 0.031)}  & \cellcolor[HTML]{c4f2cb} \new{\textbf{0.006 ($\pm$ 0.001)}}     \\ 
\multicolumn{1}{l|}{All-FT} & \cellcolor[HTML]{c4f2cb}\cellcolor[HTML]{c4f2cb} \new{\textit{\textbf{1.176 ($\pm$ 0.775)}}} %\textbf{\textit{0.703 (-93.5\%)}} 
& \cellcolor[HTML]{c4f2cb}\cellcolor[HTML]{c4f2cb} \new{\textit{\textbf{0.377 ($\pm$ 0.067)}}} %\textbf{\textit{0.401 (-52.8\%)}}   
& \cellcolor[HTML]{c4f2cb} \new{\textit{\textbf{0.013 ($\pm$ 0.002 )}}} %\textbf{\textit{0.012 (-64.4\%)}}  
& \cellcolor[HTML]{fccaca} \new{0.486 ($\pm$ 0.131)}%\textbf{0.442 (+7.6\%)} 
& \cellcolor[HTML]{fccaca} \new{\textbf{0.060 ($\pm$ 0.030)}} %\textbf{0.049 (-4.2\%)}  
& \cellcolor[HTML]{fccaca} \new{0.007 ($\pm$ 0.001)} %0.008 (+31.3\%)   
\\ \midrule 
\end{tabular}}
%\raggedright
\caption{\textbf{Closed-Loop Re-Deployment Performance.} Average robot performance metrics for each fine-tuned predictor \new{(standard deviation over three seeds of fine-tuning in parentheses)}. Two main columns are evaluations on high-regret and low-regret \new{held-out} validation scenes. Italics-bold indicates best, and bold indicates second best. Across all metrics and settings, High-regret-FT consistently improves robot performance, \new{and is competitive with the privileged All-FT approach.}}
\vspace{-1em}
\vspace{-0.25cm}

  \label{tab:CL-performance} 
\end{table*}


We compare our method, called \textbf{High-Regret-FT} which fine-tunes $\pred$ exclusively on high-regret data $\data_\mathcal{I}$ \new{containing the 17 identified high-regret scenes not held out for evaluation}, to the same predictor architecture but fine-tuned on three different 
datasets: \textbf{Random-FT} uses the randomly samples a subset \new{of 17 scenes} from the deployment data $d \sim \mathrm{Unif}[\data]$, \textbf{All-FT} uses the entire deployment dataset $\data$ \new{consisting of the 76 scenarios not held out for validation}, and \textbf{Low-Regret-FT} uses only \new{17} \new{low-regret} \new{scenarios that did not exhibit any system-level failures, sampled from} $\data \setminus \datai$. Since the last baseline does not have \textit{any} high-regret scenarios, this serves as our control the measure the impact of high-regret scenes being present in the data at all. \new{Each baseline took about 1.5 hours to finetune, except \textbf{All-FT} which took about 7 hours due to the larger dataset size. We fine-tuned each baseline across 3 independent random seeds.}

\medskip 
\noindent \textit{\textbf{Takeaway 1:} \textbf{High-Regret-FT} improves log-replay prediction accuracy in high-regret scenarios, without degrading performance on low-regret scenarios and the original Nuscenes validation set.}
\medskip 

We first evaluate the predictors ``open-loop'' on log-replay data from three different validation datasets: the original Nuscenes validation data, the 3 high-regret scenes in the deployment validation dataset, and the 17 \new{low-regret} scenes in the deployment validation dataset. 
We \new{report} the Average Displacement Error (ADE) and Final Displacement Error (FDE) \new{for each baseline's best performing seed (standard practice in the trajectory forecasting literature)} in Table \ref{tab:OL-ade-fde}. 
The base predictor (trained only on Nuscenes) doubles its ADE and FDE \new{on the simulated deployment data} due to a distribution shift in the driving behavior between Nuscenes and the simulated BITS policy. 
% This is confirmed by the fact that the ADE / FDE massively improve on both interaction-relevant and interaction-irrelevant simulation data once finetuned on any subset of the deployment data. 
Intuitively, \textbf{High-Regret-FT} reduces the ADE and FDE on high-regret validation data the most. More interestingly, it also \textit{improves} \new{open-loop prediction accuracy on low-regret scenes} over the base prediction model (\new{40}\% ADE reduction, \new{28}\% FDE reduction). 
We hypothesize this is because the \new{high-regret} validation data leaks enough information about the general distribution shift between the Nuscenes and the BITS simulation to enable a model that only saw high-regret interactions to improve on nominal \new{low-regret} interaction data as well. 
While \textbf{All-FT} achieves the best prediction accuracy across the board, it is important to note that this is an information-advantaged baseline: it has the ability to learn from both \new{system-level} and \new{non-system-level} failures the deployment data. \new{Since the amount of simulated deployment data in our experiments is quite small relative to the Agentformer prediction model's size, the model has the capacity to ``memorize'' all the deployment data.
However,} \textbf{High-Regret-FT} is fine-tuned on $77\%$ less data than \textbf{All-FT}, making it much more data efficient to train than the \textbf{All-FT} approach, while still performing the second-best in terms of quantitative metrics. 
% but its predictive capacity is only decreased by \todo{XX\% ADE / YY\% FDE reduction...}. \ttnote{What is predictive capacity?} 
As the deployment dataset $\data$ grows and training time and costs increase along with it, this can be a promising avenue to alleviate these challenges while still achieving high predictive performance.  
% The baseline using only interaction-relevant data has the second lowest ADE and FDE on the interaction-relevant validation data. 
Finally, the least amount of improvement over the base model is exhibited by \textbf{Low-Regret-FT} and followed by \textbf{Random-FT}. This is particularly important, since it demonstrates the quantitative value of attending to the high-regret interaction data. 
% The next lowest prediction error comes from the \textbf{Random-FT} baseline, which contains some instances of interaction-relevant data, and the worst prediction error on the interaction-relevant validation data comes from the baseline using only scenes deemed interaction-irrelevant by our regret metric. 

% \ttnote{I think here we also need a paragraphy to highlight our advantage in efficient training. Because training using all deployment data also gives good performance, we should highlight when we scal this is can save a lot training cost.  }
% \knnote{need to do a better job of explaining that table 1 is doing open loop prediction on log-replay data resulting from deploying the original predictor with the tree planner. closed-loop performance is evaluated on the metrics for redeploying the planner with a new predictor.}
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/qualtitative_rss24_new.png}
    \caption{\textbf{Qualitative Re-Deployment Result.} Blue robot must navigate around a new stopped truck while being mindful of other moving cars (white). Small deviations in the white vehicles are the result of inherent variation in closed-loop simulation. As the prediction model $\pred$ is targettedly re-trained on more high-regret interactions, the closed-loop performance naturally improves (top to bottom). Even though \textbf{High-Regret-FT} trains on $77\%$ less data than the \textbf{All-FT} approach, it still achieves qualitatively comparable behavior in re-deployment.}
    \vspace{-1em}
    \label{fig:qualitative}
\end{figure}

\medskip 
\noindent \textit{\textbf{Takeaway 2:} \textbf{High-Regret-FT} improves closed-loop performance metrics such as collision cost and average regret in all re-deployment scenes, even compared to \textbf{All-FT}.}
\medskip 



We use three metrics to evaluate the closed-loop re-deployment performance of our robot using each candidate fine-tuned predictor.
First, we measure \textit{Total Collision Cost}, which is the total cost the ego incurred during the simulation from collisions. 
Second, \textit{Collision Severity} which is the intensity of a collision measured by $\frac{\text{Total Collision Cost}}{\# \text{Frames in Collision}}$. This metric is used to disentangle high total collision costs resulting from 1-2 timesteps of extremely poor behavior (e.g., quickly driving through a stopped vehicle) versus many timesteps of small collision costs (e.g., stopped bumper-to-bumper at an intersection). Finally, we measure average \textit{Regret} as defined in Section \ref{sec:method-failure-detection}. \new{We report the average closed-loop performance for each method across three seeds of fine-tuning in Table \ref{tab:CL-performance}}.

% The closed-loop performance on interaction-irrelevant data has very small changes compared to the changes in the task-relevant data performance.
We find that \textbf{High-Regret-FT} decreases collision cost, severity, and average regret compared to the base model across both \new{high-} and \new{low-regret} scenes. As hypothesized, most closed-loop performance gains are observed in the \new{high-regret} scenes, decreasing robot regret by $-\new{53}\%$ and collision cost by $-\new{65}\%$ (shown in Table~\ref{tab:CL-performance}). 
By being able to see all the deployment data, \textbf{All-FT} observes the highest performance gains in \new{high-regret} scenes but shows performance degradation in \new{low-regret} scenes (increasing robot regret by about $+31\%$ and collision cost by $+7\%$). \new{However, we note that the performance degradation in low-regret scenarios is not statistically significant. For each baseline, the results from the baseline model are within 1 standard deviation (except for the regret of \textbf{Low-Regret-FT}). In contrast, the improved performance of \textbf{High-Regret-FT} is more than one standard deviation better than the performance of \textbf{Low-Regret-FT} and \textbf{Random-FT} with respect to the collision-based metrics.} 

%We hypothesize that this phenomenon emerges from deployment dataset imbalance; %\textcolor{red}{as discussed in Takeaway 4 below}, the low-regret data that dominates $\data$ can unintuitively degrade the planner's ability to understand key human behaviors (as observed by the performance of \textbf{Low-Regret-FT}. \todo{change this paragraph, degradation is not statistically significant}.


\medskip 
\noindent \textit{\textbf{Takeaway 3:} Closed-loop and open-loop performance are only correlated on high-regret scenes.}%; prediction error on other scenes can be arbitrarily bad.} 
\medskip 

% We find that ``open-loop'' prediction performance can be an inconsistent indicator of closed-loop robot performance.
% Specifically, we observed that open-loop perfomance \textit{improvements} can lead to signifigantly \textit{worse} closed-loop performance in the \new{low-regret} scenes 
% (e.g., 34\% ADE improvement from \textbf{Low-Regret-FT} in Table~\ref{tab:OL-ade-fde} corresponds to around 80\% degredation in all closed-loop metrics in Table~\ref{tab:CL-performance}).

We find that in the \new{high-regret} scenes, the open-loop performance (Table~\ref{tab:OL-ade-fde}) is positively correlated with the closed-loop planner performance (Table~\ref{tab:CL-performance}). 
We hypothesize that this is because these scenes are much more challenging (e.g., highly interactive), encode more nuanced human behavior, and affect the planner the most; thus, the prediction improvements in such scenarios indicate that $\pred$ has learned to capture interaction better which naturally improves the planning performance.
%\todo{again, degradation is not statistically significant}



\section{\new{Preliminary Results: Detecting Interaction Failures of Generative Planners}}

One consequence of our likelihood-based approach is that it generalizes a notion of calibrated regret to be readily compatible with generative neural planners. \new{These neural planners learn a joint distribution of multi-agent behavior and execute the most likely ego plan under the joint distribution \cite{luo2022jfp, seff2023motionlm}. However, this means that they do not maintain explicit rewards, prohibiting the application of prior system-level anomaly detection methods \cite{farid2023task}.}
%Here, the conditional probability $P_\phi$ can be naturally approximated via querying the generative planner \cite{seff2023motionlm}. 
With the rise of these types of models in robotics, we see this as an important step towards uniting core decision-theoretic concepts with increasingly powerful but opaque planning paradigms. 

\new{To substantiate the generality of our metric across both application domains and type of planner, we further demonstrate 
% the ability of 
how our regret metric can automatically identify system-level prediction failures when the robot's planner is a generative model in a simulated social navigation setting. }

\new{\para{Setup} The robot is modeled as a Dubins' car dynamical system \cite{dubins} and is tasked with reaching a goal while navigating around a planar pedestrian that can freely move in any direction.
The robot is given one of two goals $g_R \in \{\texttt{top}, \texttt{right}\}$ and is allowed to observe an initial low-dimensional behavior cue of the human (e.g., eye gaze, head tilt) denoted by $\delta_\human$. The robot must reach its intended goal unless it predicts that doing so will intersect with the human's predicted path; in this case, the robot switches to navigate to the other goal (Figure~\ref{fig:generative-main}). The robot's generative planner $\plan(\cdot)$ is a Vector-quantized Variational Autoencoder (VQ-VAE) \cite{van2017neural} trained on simulated multi-agent interaction data described below. 

\para{Dataset Generation} We constructed a dataset of $|\data_{train}| = 10,000$ human-robot trajectories based on a small set of simple rules in order to train our generative planner. The positions of the two goal locations and the robot and human's start locations were fixed in all training examples (shown in Figure \ref{fig:generative-main}), but the choice of goal $g$ and initial human behavior cue $\delta_\human$ were uniformly distributed.
The synthetic human trajectory generation abides by the following rule: $\aHOnetraj = PC(\texttt{left})$ if $\delta_H + \epsilon < 1/3$, $PC(\texttt{right})$ if $\delta_\human + \epsilon> 2/3$, $PC(\texttt{down})$ otherwise. Here, $PC(\cdot)$ denotes a proportional controller noisily executing a 6-timestep action trajectory that guides the human to the prespecified goal points to the left, right, or below the human's initial position, and $\epsilon$ is zero-mean noise.   %modeling the human as choosing a high-level behavior primitive, $u_\human \in \{\texttt{left}, \texttt{right}, \texttt{down}\}$, informed by their current behavior cue $\delta_\human$. 
%Specifically, 
% Based on the heading $\theta_\human$ of the human, 
%we sample $\bar{\delta}_\human \sim \mathcal{N}(\delta_\human, \sigma^2_\human)$ where $\sigma^2_\human$ was set to 0.2, and the human's high-level behavior primitive is determined by
% that determined the human's high-level behavior $u_\human$. 
%$u_\human = \texttt{left}$ if $\bar{\delta}_\human < \frac{1}{3}$, $u_\human = \texttt{right}$ if $\bar{\delta}_\human > \frac{2}{3}$, and $u_\human = \texttt{down}$ otherwise. 
%Finally, the high-level primitive $u_\human$ determines a 6-timestep action trajectory that was noisily executed by the simulated human, and is denoted as $\aHOnetraj$.

The synthetic robot trajectory generation follows a similar process, but conditions on the desired goal $g_R$ and the synthetic human behavior  $\aHOnetraj$. %The robot's behavior primitive, $u_\robot$, steers the robot directly to its goal ($u_\robot = g$) if it did not lead to colliding with the human (e.g., $g = \texttt{top}$ and $u_\human \neq \texttt{down}$). 
The robot's action $\aRtraj$ is a noisily executed 6-timestep action trajectory given by a proportional controller that guides the robot to $g_R$, unless this brings the robot in close proximity to the human trajectory $\aHOnetraj$ in which case the robot's proportional controller guides it to the other goal with 80$\%$ probability.
%In the event that going to the goal leads to a collision with the human, the robot would sample a new goal location where it switches to the other goal with 80$\%$ probability ($u_\robot \neq g$) and stays with the current goal otherwise.
% and went to the queried goal otherwise. 
%Given a choice of $u_\robot$, the robot executed a 6-timestep action trajectory $\aRtraj$ by following a proportional controller injected with Gaussian noise to reach the goal specified by $u_\robot$. 
This dataset synthesis leads to six different high-level outcomes of the interaction depending on which directions the human and robot travel. %joint human-robot behavior primitives given by the Cartesian product of $u_\robot \in \{\texttt{top}, \texttt{right}\}$ and $u_\human \in \{\texttt{left}, \texttt{down}, \texttt{right}\}$. 
Figure \ref{fig:generative-main} shows three of these joint human-robot interaction outcomes.

\para{Generative Planner Architecture} The robot's generative planner $\plan$ predicts the joint distribution of future human-robot behavior conditioned on the robot's observation and the robot's goal. 
% To generate such joint human-robot motion plans, 
We used an encoder-decoder architecture based on the VQ-VAE, which is a variant of the traditional VAE that uses vector quantization to discretize the latent representation into $K$ latent embedding vectors $\{ z_k\}_{k=1}^K$. 
The encoder $P_\alpha(z \mid \delta_\human, g)$ with learnable parameters $\alpha$ takes $\delta_\human$ and $g_R$ as inputs to encode the input and produce a categorical distribution over latent embedding through vector quantization. We further inject a small amount of zero-mean Gaussian noise into quantized embedding $z \in \{ z_k\}_{k=1}^K$ to encourage diverse outputs during the joint trajectory decoding phase.
This decoder $P_\beta(\aRtraj, \aHOnetraj \mid z)$ with learnable parameters $\beta$ takes a sampled latent vector $z$ as input (sampled from $P_\alpha(z \mid \delta_\human, g)$ with additional noise injection) to approximate the joint distribution over actions $\aRtraj, \aHOnetraj$. In our setting, we set $K = 6$ and initialized the latent embeddings with K-means clustering to encourage each of the K embedding vectors to correspond to one of the six joint human-robot action trajectories.




%The encoder, embedding vectors, and decoder are all jointly trained. We modify the traditional VQ-VAE architecture such that the sampled quantized embedding $z \in \{ z_k\}_{k=1}^K$ is injected with a small amount of zero-mean Gaussian noise prior to decoding in order to encourage diversity in the reconstructed joint human-robot trajectories. 
%This noise-injected decoder is denoted as $P_\beta(\aRtraj, \aHOnetraj \mid z)$ with learnable parameters $\beta$; note that we can sample from this probability density function, but we do not have an analytic expression for it.
%In our setting, we set $K = 6$ and initialized the latent embeddings with K-means clustering to encourage each of the K embedding vectors to correspond to one of the six joint human-robot action trajectories. 

%In order to sample from $\plan$, we also learned a conditional VQ-VAE prior over behavior primitives, $P_\alpha(z \mid \delta_\human, g)$, with learnable parameters $\alpha$ that takes $\delta_\human$ and $g_R$ as inputs to generate a categorical distribution over latent embedding. The sampling process consists of first sampling the latent joint-interaction embedding from the prior $P_\alpha(z \mid \delta_\human, g_R)$, and then generating the low-level actions $\aRtraj, \aHOnetraj$ by querying the decoder, $P_\beta$.

By designing the generative planner in this way, it is straightforward to generate action trajectories conditioned on not only the robot's observation and goal but also sample action trajectories conditioned on one of the six high-level interaction outcomes. This generative model does planning and prediction simultaneously conditioned on the state $\state_t = \delta_\human$ and context $\context = g_R$ and connects to the policy $\pi_\phi$ and predictor $\pred$ as defined in Section \ref{sec:problem-formulation} where the neural network weights of the policy and predictor are equivalent (i.e., $\theta \equiv \phi$) and specifically consist of $\alpha$ and $\beta$.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/RSS24CalibratedRegret-Gen.png}
    \caption{\new{\textbf{Our Regret Metric with a Generative Planner.} Even when using a generative model for joint planning and prediction, our generalized regret metric can correctly detect poor behavior. (left) Human behaved as predicted, and the robot incurred low regret. (middle) The robot mispredicted the human's behavior, but the robot's actions were still likely under the ground-truth joint behavior and incurred low regret. (right) The robot mispredicted the human's behavior in a way that led to a low-probability human-robot joint trajectory and incurred high regret.}}
    \label{fig:generative-main}
\end{figure}

\para{Calibrated Regret Computation} Since the behavior cue $\delta_\human$  does not solely determine $\aHOnetraj$, it is possible that the generative planner mispredicts the human's executed actions and thus executes a poor plan. 
Suppose the robot samples latent embedding $\tilde{z}$ from $P_\alpha$ and conditions on this to generate the joint action trajectory $\tilde{\bm{a}}_\robot, \tilde{\bm{a}}_\human$ from $P_\beta$. 
The robot's executed trajectory is precisely this action trajectory, $\aRtrajObs := \tilde{\bm{a}}_\robot$; however, the ground-truth trajectory of the human, $\aHOnetrajObs$, may not be aligned with the original action trajectory that the robot anticipated ($\tilde{\bm{a}}_\human$).
% \tilde{a}_\human$, then we must evaluate the quality of the robot's action $\hat{a}_\robot$. 

Recall that our regret computation in Equation~\ref{eq:regret} hinges on evaluating the likelihood of executed robot decisions given the true human behavior and the most likely hindsight decision. To perform this computation, we must first obtain the counterfactual conditional probability density of the robot's trajectory: $P(\aRtrajObs \mid \aHOnetrajObs, \delta_\human, g)$. 
We leverage our ability to sample from the decoder $P_\beta$ to form a kernel density estimate of $P_\beta(\aRtrajObs, \aHOnetrajObs  \mid \tilde{z})$ by querying the decoder 100 times. 
We then approximate the conditional probability of $\aRtrajObs, \aHOnetrajObs$ by integrating the KDE around a small neighborhood of the ground-truth joint action trajectory. Furthermore, the conditional probability of $\aHOnetrajObs$ can be approximated by marginalizing over all possible $\aRtraj$. %integrating the KDE over all possible $\aRtraj$.
Leveraging the approximate probabilities, we compute the counterfactual probability for any $\aRtrajObs$
\begin{equation*}
\small
\begin{aligned}
    &P(\aRtrajObs \mid \aHOnetrajObs, \delta_\human, g_\robot) = \\ 
    &\quad\quad\quad \frac{\sum_{z}P_\beta(\aRtrajObs, \aHOnetrajObs \mid z) P_\alpha(z \mid \delta_\human, g_\robot)}{\int_{\tilde{\bm{a}}_\robot}\sum_{z}P_\beta(\aHOnetrajObs, \tilde{\bm{a}}_\robot, \mid z) P_\alpha(z \mid \delta_\human, g_\robot)}.
\end{aligned}
\end{equation*}
\normalsize
Note that this is a particular instantiation of \eqref{eq:cfprob} where the planner and predictor parameters are the same ($\phi \equiv \theta$) and are parameterized by $\alpha$ and $\beta$; we then compute the desired probability using Bayes' theorem. 
We repeat this process for the maximum probability action trajectory $\aRtraj$\footnote{In practice, finding this maximizing $\aRtraj$ is approximated by searching over a prespecified set of action trajectories.} to compute our regret metric from Equation~\ref{eq:regret}.

\para{Results} The results of the regret metric in the generative planning domain are shown in Figure \ref{fig:generative-main}.
Our regret metric only flags interactions as anomalous when mispredictions lead to unexpectedly close proximity interactions between the robot and human (right, Figure~\ref{fig:generative-main}).
In both nominal interactions (left, Figure~\ref{fig:generative-main}) and interactions where mispredictions did not lead to close-proximity interactions (center, Figure~\ref{fig:generative-main}), the deployment regret is quite low. 
Importantly, we highlight that our generalized calibrated regret metric captures the intuition on what is a system-level prediction failure without the need for manually specifying an evaluative reward-function for either the high-level or low-level robot and human behaviors.}



%\todo{FINISH THIS!}


%\medskip 
%\noindent \textit{\textbf{Takeaway 4:} \textbf{Low-Regret-FT} degrades overall planner performance.}
%\medskip 

%Although \textbf{Low-Regret-FT} improved the predictor's ``open-loop'' performance in both interaction-relevent and interaction irrelevent scenes, this improvement did not extend to closed-loop simulation. Instead, \textbf{Low-Regret-FT} leads to closed-loop degradation, even in the interaction-irrelevant scenarios on which the predictor was fine-tuned. 
%\todo{We hypothesize that this is because fine-tuning $\pred$ only on interaction-irrelevent scenarios degrades the model's original ability to understand human behavior impacting downstream planning.}
%This is especially undesirable because most of the scenarios that the robot will encounter in deployment-time are actually interaction-irrelevent. 


% \begin{table*}[bth]
% \centering
% \caption{Closed-loop Deployment: Task-relevant}
%   \begin{tabular}{lllllllll}
% \toprule
%  \cellcolor[HTML]{D7D7D7} Finetuning Method & $\Delta$Total Collision Cost & $\Delta$Collision Severity & $\Delta$Average Regret   \\ \midrule

% \multicolumn{1}{l|}{Highest-regret (ours)} 
% & -60.4\% (-6.541)
%   & -18.7\% (-0.159)
%   & -58.7\% (-0.020)
%       \\ 
% \multicolumn{1}{l|}{Random}            
% & -42.6\% (-4.614)

%            & -13.9\% (-0.118)
%          &  -58.7\% (-0.020)

%             \\
% \multicolumn{1}{l|}{All} & -93.5\% (-10.125)
% &-52.8\% (-0.448)
%   & -64.4\% (-0.022)
%   \\
% \multicolumn{1}{l|}{Lowest Regret} & -32.0\% (-3.464)
% & +0.8\% (+0.07)
%   & -44.2\% (-0.015)
%     \\ \midrule
% \end{tabular}

% Percent change in average performance differences between different fine-tuning methods compared to the original base predictor. Absolute mean difference in parentheses.
%   \label{tab:2}
% \end{table*}


% \begin{table*}[t]
% \centering
% \caption{Closed-loop Deployment: Task-irrelevant}
%   \begin{tabular}{lllllllll}
% \toprule
%  \cellcolor[HTML]{D7D7D7} Finetuning Method & $\Delta$Total Collision Cost & $\Delta$Collision Severity & $\Delta$Average Regret   \\ \midrule

% \multicolumn{1}{l|}{Highest-regret (ours)} 
% & -15.5\% (-0.064)
%   & -24.9\% (-0.013)
%   & -11.1\% (-0.001)
%       \\ 
% \multicolumn{1}{l|}{Random}            
% & +0.8\% (+0.329)

%            & +1.7\% (+0.087)
%          &  +0.1\% +( 0.000)

%             \\
% \multicolumn{1}{l|}{All} & +7.6\% (+0.031)
% &-4.2\% (-0.002)
%   & +31.3\% (+0.002)
%   \\
% \multicolumn{1}{l|}{Lowest Regret} & +106.4\% (+0.437)
% & 80.6\% (+0.041)
%   & +54.5\% (0.003)
%     \\ \midrule
% \end{tabular}







% \para{Qualitative Results}

% \todo{\textbf{Takeaway 1 [open-loop results]}: “After fine-tuning, our model can learn to predict interactions that were identified as task-relevant failures by our regret metric.”

% \textbf{Takeaway 2 [open-loop results]}: “Fine-tuning only on task-relevant data also improves prediction accuracy on task-irrelevant data.” => hypothesis: this is because the task-relevant data also leaks information about general distribution shift from the nuScenes training data to the TB Sim deployment data distribution.

% \textbf{Takeaway 3 [closed-loop results]}: “Fine-tuning the predictor on task-relevant data improves closed-loop performance. Specifically, the robot’s collision frequency and avg/worst-case regret is decreased upon re-deployment in scenarios where task-relevant failures occurred.”

% \textbf{Takeaway 4 [Open and closed-loop results]}: “Closed-loop and open-loop performance are only correlated on interaction-relevant scenes; prediction error on other scenes can be arbitrarily bad” \knnote{wrote this down but might be paradoxical... we call it an interaction relevant scene bc bad predictions lead to bad interactions. think ab this more}}


